Device-Aware Routing and Scheduling in Multi-Hop Device-to-Device Networks

The dramatic increase in data and connectivity demand, in addition to heterogeneous device capabilities, poses a challenge for future wireless networks. One of the promising solutions is Device-to-Device (D2D) networking. D2D networking, advocating the idea of connecting two or more devices directly without traversing the core network, is promising to address the increasing data and connectivity demand. In this paper, we consider D2D networks, where devices with heterogeneous capabilities including computing power, energy limitations, and incentives participate in D2D activities heterogeneously. We develop (i) a device-aware routing and scheduling algorithm (DARS) by taking into account device capabilities, and (ii) a multi-hop D2D testbed using Android-based smartphones and tablets by exploiting Wi-Fi Direct and legacy Wi-Fi connections. We show that DARS significantly improves throughput in our testbed as compared to state-of-the-art.

==> refs.tex <==

\bibliographystyle{IEEEtran}
%\vspace{-5pt}
\begin{thebibliography}{}
%\vspace{-5pt}
%\scriptsize

\bibitem{cisco_index} Cisco Visual Networking Index: Global Mobile Data Traffic Forecast Update, 2010 - 2015.

\bibitem{ericsson_report} Ericsson Mobility Report, November 2013.

%\bibitem{solar_case} http://www.mobiletechreview.com/ubbthreads/showflat.php?Number=41450

%\bibitem{solar_battery} http://www.mobiletechreview.com/ubbthreads/showflat.php?Number=40821

\bibitem{microcast} L.~Keller, A.~Le, B.~Cici, H.~Seferoglu, C.~Fragouli, A.~Markopoulou, ``MicroCast: Cooperative Video Streaming on Smartphones'' {\em in Proc. of ACM MobiSys}, Low Wood Bay, Lake District, UK, June 2012.

\bibitem{microcast_allerton} H.~Seferoglu, L.~Keller, B.~Cici, A.~Le, A.~Markopoulou,``Cooperative Video Streaming on Smartphones'' {\em in Proc. of Allerton}, 2011.

\bibitem{tutorial_lin} X. Lin, N. B. Schroff, R. Srikant, ``A tutorial on cross-layer optimization in wireless networks,'' {\em in IEEE JSAC}, vol. 24(8), Aug. 2006.

\bibitem{tutorial_doyle} M.~Chiang, S.~T.~Low, A.~R.~Calderbank, J.~C.~Doyle, ``Layering as optimization decomposition: a mathematical theory of network architectures,'' \emph{in Proceedings of the IEEE}, vol.~95(1), Jan. 2007.


%\bibitem{thisTechRep} H.~Seferoglu, Y.~Xing, ``Device-Centric Cooperation in Mobile Networks,'' Tech. Report, available at {\em http://www.mit.edu/{\texttildelow}hseferog/}.

%\bibitem{micro1} S.~Ioannidis, A.~Chaintreau, L.~Massoulie, ``Optimal and scalable distribution of content updates over a mobile social network,'' {\em in Proc. of INFOCOM}, Rio de Janeiro, Brazil, Apr. 2009.
%
%\bibitem{micro2} B.~Han, P.~Hui, V.~A.~Kumar, M.~V.~Marathe, G.~Pei, A.~Srinivasan, ``Cellular traffic offloading through opportunistic communications: a case study,'' {\em in Proc. of ACM Workshop on Challenged Networks (CHANTS)}, Chicago, IL, Sept. 2010.
%
%\bibitem{micro3} J.~Whitbeck, M.~Amorim, Y.~Lopez, J.~Leguay, V.~Conan, ``Relieving the wireless infrastructure: When opportunistic networks meet guaranteed delays,'' {\em in Proc. of IEEE WoWMoM}, Lucca, Italy, June 2011.
%
%\bibitem{micro4} P.~Hui, J.~Crowcroft, E.~Yoneki, ``Bubble rap: social-based forwarding in delay tolerant networks,'' {\em in Proc. of ACM MobiHoc}, Hong Kong, May 2008.
%
%\bibitem{micro5} C.~Boldrini, M.~Conti, A.~Passarella, ``Exploiting users' social relations to forward data in opportunistic networks: The HiBOp solution,'' {\em in Proc. of Pervasive and Mobile Computing}, Oct. 2008.
%
%
%\bibitem{micro6} M.~Ramadan, L.~El Zein, Z.~Dawy, ``Implementation and evaluation of cooperative video streaming for mobile devices,'' {\em in Proc. of IEEE PIMRC}, Cannes, France, Sept. 2008.
%
%\bibitem{micro7} S. Li and S. Chan, ``BOPPER: wireless video broadcasting with peer-to-peer error recovery,'' {\em in Proc. of IEEE ICME}, Beijing, China, July 2007.

\bibitem{prop11} S. Ioannidis, A. Chaintreau, and L. Massoulie, ``Optimal and scalable distribution of content updates over a mobile social network,'' {\em in Proc. IEEE INFOCOM}, Rio de Janeiro, Brazil, April 2009.

\bibitem{prop12} B. Han, P. Hui, V. A. Kumar, M. V. Marathe, G. Pei, and A. Srinivasan, ``Cellular traffic offload- ing through opportunistic communications: a case study,'' {\em in Proc. of ACM Workshop on Challenged Networks (CHANTS)}, Chicago, IL, September 2010.

\bibitem{prop13} J. Whitbeck, M. Amorim, Y. Lopez, J. Leguay, and V. Conan, ``Relieving the wireless infrastructure: When opportunistic networks meet guaranteed delays,'' {\em in Proc. of IEEE WoWMoM}, Lucca, Italy, June 2011.

\bibitem{prop14} P. Hui, J. Crowcroft, and E. Yoneki, ``Bubble rap: social-based forwarding in delay tolerant networks,'' {\em in Proc. of ACM MobiHoc}, Hong Kong, May 2008.

\bibitem{prop15} C. Boldrini, M. Conti, and A. Passarella, ``Exploiting users’ social relations to forward data in opportunistic networks: The hibop solution,'' {\em in Proc. of Pervasive and Mobile Computing}, October 2008.

\bibitem{prop7} M.Ramadan, L.E.Zein, and Z.Dawy, ``Implementation and evaluation of cooperative video streaming for mobile devices,'' {\em in Proc. of IEEE PIMRC}, Cannes, France, September 2008.

\bibitem{prop8} S. Li and S. Chan, ``Bopper: wireless video broadcasting with peer-to-peer error recovery,'' {\em in Proc. of IEEE ICME}, Beijing, China, July 2007.

\bibitem{prop16} C. Tsao and R. Sivakumar, ``On effectively exploiting multiple wireless interfaces in mobile hosts,'' {\em in Proc. of ACM CoNEXT}, December 2009.

\bibitem{prop17} H. Soroush, P. Gilbert, N. Banerjee, M. D. Corner, B. N. Levine, and L. Cox, ``Spider: improving mobile networking with concurrent wi-fi connections,'' {\em SIGCOMM CCR}, vol. 41, no. 4, August 2011.

\bibitem{prop18} P. Rodriguez, R. Chakravorty, J. Chesterfield, I. Pratt, and S. Banerjee, ``Mar: a commuter router infrastructure for the mobile internet,'' {\em in Proc. of ACM MobiSys}, June 2004.

\bibitem{prop19} J.Chesterfield, R.Chakravorty, I.Pratt, S.Banerjee, and P.Rodriguez, ``Exploiting diversity to enhance multimedia streaming over cellular links,'' {\em in Proc. of IEEE INFOCOM}, March 2005.

\bibitem{prop20} J.Chesterfield, R.Chakravorty, I.Pratt, S.Banerjee, and P.Rodriguez, ``A system for peer-to-peer video streaming in resource constrained mobile environments,'' {\em in Proc. of ACM U-NET}, December 2009.

\bibitem{prop21} G. Ananthanarayanan, V. N. Padmanabhan, L. Ravindranath, and C. A. Thekkath, ``Combine: leveraging the power of wireless peers through collaborative downloading,'' {\em in Proc. of ACM MobiSys}, June 2007.

%\bibitem{micro8} J. B. Saleh, D. Qiu, and A. K. Elhakeem, ``Performance of an efficient scheduling approach to network coding for wireless local repair,'' {\em Cyber Journals: Journal of Selected Areas in Telecommunications (JSAT)}, vol. 2, no. 1, pp. 49�58, Jan. 2011.

%\bibitem{micro9} M. Pedersen and F. Fitzek, ``Implementation and performance evaluation of network coding for cooperative mobile devices,'' {\em in Proc. of IEEE ICC}, May 2008.

%\bibitem{micro10} M. Pedersen, J. Heide, F. Fitzek, and T. Larsen, ``PictureViewer - a mobile application using network coding,'' {\em in Proc. of European Wireless Conference}, May 2009.

%\bibitem{micro11} P. Vingelmann, M. Pedersen, F. Fitzek, and J. Heide, ``On-the-fly packet error recovery in a cooperative cluster of mobile devices,'' {\em in Proc. of IEEE GLOBECOM}, Dec. 2011.

%\bibitem{book_srikant} R.~Srikant, ``The mathematics of Internet congestion control'', Birkhauser, 2003.


\bibitem{gupta_interference_model} P.~Gupta, P.~R.~Kumar, ``The capacity of wireless networks,'' \emph{in IEEE Trans. on Information Theory}, vol.~34(5), 2000.

\bibitem{dash} ISO/IEC JTC1/SC29/WG11, ``Information technology - Dynamic adaptive streaming over HTTP (DASH) -- Part 1: Media presentation description and segment formats'', ISO/IEC 23009-1:2012, 2012.

\bibitem{netflixdash} http://techblog.netflix.com/2010/12/html5-and-video-streaming.html

\bibitem{tass1} L. Tassiulas, A. Ephremides, ``Stability properties of constrained queueing systems and scheduling policies for maximum throughput in mul- tihop radio networks,'' {\em in IEEE Trans. on Automatic Control}, vol. 37(12), Dec. 1992.

\bibitem{tass2} L. Tassiulas and A. Ephremides, ``Dynamic server allocation to parallel queues with randomly varying connectivity,'' {\em in IEEE Trans. on Information Theory}, vol. 39(2), March 1993.

\bibitem{neelymoli} M. J. Neely, E. Modiano, and C. Li, ``Fairness and optimal stochastic control for heterogeneous networks,'' {\em in IEEE/ACM Trans. on Networking}, vol. 16(2), April 2008.

\bibitem{limod} C.-P.~Li and E.~Modiano, ``Receiver-Based Flow Control for Networks in Overload,'' {\em in IEEE/ACM Transactions on Networking}, 2014.

\bibitem{neelybook} M.~J.~Neely, ``Stochastic network optimization with application to communication and queueing systems,'' Morgan \& Claypool, 2010.


\end{thebibliography}
